Revealing Personality Traits: A New Benchmark Dataset for Explainable Personality Recognition on Dialogues

Personality recognition aims to identify the personality traits implied in user data such as dialogues and social media posts. Current research predominantly treats personality recognition as a classification task, failing to reveal the supporting evidence for the recognized personality. In this paper, we propose a novel task named Explainable Personality Recognition, aiming to reveal the reasoning process as supporting evidence of the personality trait. Inspired by personality theories, personality traits are made up of stable patterns of personality state, where the states are short-term characteristic patterns of thoughts, feelings, and behaviors in a concrete situation at a specific moment in time. We propose an explainable personality recognition framework called Chain-of-Personality-Evidence (CoPE), which involves a reasoning process from specific contexts to short-term personality states to long-term personality traits. Furthermore, based on the CoPE framework, we construct an explainable personality recognition dataset from dialogues, PersonalityEvd. We introduce two explainable personality state recognition and explainable personality trait recognition tasks, which require models to recognize the personality state and trait labels and their corresponding support evidence. Our extensive experiments based on Large Language Models on the two tasks show that revealing personality traits is very challenging and we present some insights for future research. Our data and code are available at https://github.com/Lei-Sun-RUC/PersonalityEvd.

==> sub_modules/Rebuttal.tex <==
\clearpage
\section{Reviewer EnFY}
\subsection{Score}
Overall Assessment:3 Soundness:3 Confidence:4
\subsection{Strength}
This paper is well structured and described. It provides a very clear flow of the dataset construction process and has evaluated the contribution of including the short-term personality state task towards the better performance on the long-term personality trait recognition.
\subsection{Weakness}
The proposed dataset is small-scale. Though the reason is briefly mentioned in the limitation section, it would be more convincing to include the time and costs of the annotations for the current dataset.

\subsection{Comments Suggestions And Typos}
It could be interesting to see how accurate the GPT-4 pre-annotations are and roughly how many instances are corrected by the manual annotators afterwards. It would also be nice to know why the personality state task annotations have no supporting evidence in terms of the combination of three-faceted descriptions, e.g. anxiety/depression/emotional volatility in neuroticism.
\subsection{Reply}


\section{Reviewer 5A3r}
\subsection{Score}
Overall Assessment:4 Soundness:3.5 Confidence:4
\subsection{Strength}
Computational approaches to personality focus on identifying categorical labels for personality types. When reasoning has been applied to these classifiers, they typically utilize approaches like LIME (Ribeiro et al., 2016), which utilize the lexical evidence for and against categories.
The authors approach here is novel, leveraging Chain of Thought Prompting for explaining decisions behind a text classifier. It has the potential to provide better reasoning for text classification in a human readable/understandable text description, behind just personality identification.
\subsection{Weakness}
The dataset was constructed around scripted actors portraying characters, and not in a natural environment. The personality dataset is affected by how well the scriptwriters wrote the characters, how well and how consistent actors portrayed their character, as well as the skill and determination of the directors and the post-editing technicians. Because of this, I feel the dataset and any software derivatives would be highly constrained to the entertainment domain. This may be the intended use by the authors, but I wanted to point out to the authors their Chain of Personality Evidence technique may have more impact on the field if they reproduce their annotation approach with a dataset of naturally produced language.

As the dataset was constructed around actors/characters, standardized and psychometrically validated personality tests or self-report questionnaires were not/could not be applied. Personality psychologists and computational social scientists may feel this is a limitation, as personality categorization typically utilizes the subject’s input. In addition, validated personality tests could provide objective evidence for the generated explanations.

\subsection{Comments Suggestions And Typos}
While an interesting technique that I think could be important, useful, and could extend beyond personality identification, I don't know why the technique was demonstrated on this data. In order for me to trust the technique, I feel I would need to see it evaluated on a more traditional personality dataset.
The authors may be interested in

Hannah, Domino, Hanson, Hannah (1994). Acting and Personality Change. The measurement of Change in Self-Perceived Personality Characteristics during the Actor’s Character Development Process. Journal of Research in Personality (28) 277-286.

Greene and Weiner. (2017) Handbook of Personality Assessment (2nd Ed.) Wiley.

\subsection{Reply}


\section{Reviewer EnFY}
\subsection{Score}
Overall Assessment:3 Soundness:2.5 Confidence:3
\subsection{Strength}
1. The novelty and relevance of the introduced task of explainable personality recognition.
2. The introduction of a novel dataset for the aforementioned tasks (~2K dialogueues and 72 speakers).
3. The paper is well structured and well written, generally easy to follow.
\subsection{Weakness}
1. The main concern is in the use of GPT-4 for the pre-annotation. While it is becoming common practice to use LLMs in order to reduce annotation costs, the paper lacks an analysis of the impact of using GPT-4 for pre-annotating the dataset. How much does it influence the annotation conducted by humans? I.e., how much differ the annotations when pre-annotated by GPT-4 and then corrected by humans versus human generated from scratch?

2. Lines 278-284: It is unclear how employing GPT-4 to pre-annotate solves the need of “a multi-perspective understanding of the dialogueue”.

3. Lines 286-288 “GPT-4 exhibits strong performance on various tasks, including the personality and explanation task”: How was this evaluated? Could you add a reference supporting your statement?

4. Some unclarities in the annotation process: (4a) Lines 324-327: Who are the quality inspectors? Are they taken from the 12 undergraduates? (4b) Did the quality inspectors split the instances, or are they both reviewing all of them? So, do you have 2 or 3 annotators per instance? (4c) Who does the final check (who is “we” in lines 333 and 369)? If it refers to the authors, what is the background? I recommend adding the dataset statement in the appendix with information about all the annotators (Bender and Friedman, 2018). (4d) Lines 359-361: After GPT-4, one annotator, one (or two) quality inspector, and an additional final check (from the authors), how likely is it that “the original annotation is unreasonable”? How often does it happen, do you have any statistics of how many instances got modified at this second stage?

5. The use of LLMs for evaluating the natural language reasoning process is not well motivated and is not evaluated. What are the models measuring? How are the scores reported by these models reliable, and how should we interpret them? Have you performed some qualitative or quantitative evaluation of the use of these models for measuring the similarity between two texts?

\subsection{Comments Suggestions And Typos}
1. I think it would be relevant to add TwiSty (Verhoeven et al., 2016) in your related work.

2. It could be interesting to add the standard deviations of the averages in Table 1.
Ben Verhoeven, Walter Daelemans, and Barbara Plank. 2016. TwiSty: A Multilingual Twitter Stylometry Corpus for Gender and Personality Profiling. In Proceedings of the Tenth International Conference on Language Resources and Evaluation (LREC'16), pages 1632–1637, Portorož, Slovenia. European Language Resources Association (ELRA).
\subsection{Reply}

\clearpage
